EgoMAGIC- An Egocentric Video Field Medicine Dataset for Training Perception Algorithms

This paper introduces EgoMAGIC (Medical Assistance, Guidance, Instruction, and Correction), an egocentric medical activity dataset collected as part of DARPA's Perceptually-enabled Task Guidance (PTG) program. This dataset comprises 3,355 videos of 50 medical tasks, with at least 50 labeled videos per task. The primary objective of the PTG program was to develop virtual assistants integrated into augmented reality headsets to assist users in performing complex tasks. To encourage exploration and research using this dataset, the medical training data has been released along with an action detection challenge focused on eight medical tasks. The majority of the videos were recorded using a head-mounted stereo camera with integrated audio. From this dataset, 40 YOLO models were trained using 1.95 million labels to detect 124 medical objects, providing a robust starting point for developers working on medical AI applications. In addition to introducing the dataset, this paper presents baseline results on action detection for the eight selected medical tasks across three models, with the best-performing method achieving average mAP 0.526. Although this paper primarily addresses action detection as the benchmark, the EgoMAGIC dataset is equally suitable for action recognition, object identification and detection, error detection, and other challenging computer vision tasks. The dataset is accessible via zenodo.org (DOI: 10.5281/zenodo.19239154).

==> figures/helmet_fig.tex <==
%%v-------------------------------------------------------------------v
%
%  All Sensors Performance Table
%
\begin{figure}[hb]
  %%%
  \centering
  \includegraphics[width=0.6\columnwidth]{figures/helmet.png}

  \caption{
    Picture of data collection helmet.  A Zed 2i is connected to a Nvidia Jetson Nano along with an external battery pack.}
  \label{fig:helmet}
\end{figure}
%
%%^-------------------------------------------------------------------^

==> figures/results/perf.tex <==
%%v-------------------------------------------------------------------v
%
%  Performance Plots
%
\begin{figure*}[ht]
  %%%
  \centering
    \includegraphics[width=1\textwidth]{figures/results/perf.png}
  \caption{
    Performance results for the 8 selected trauma skills.}
  \label{fig:perf}
\end{figure*}
%
%%^-------------------------------------------------------------------^

==> figures/skills_figure/skills1.tex <==
%%v-------------------------------------------------------------------v
%%v-------------------------------------------------------------------v
%
\begin{figure*}[!htb]
\centering
%%%%%%%%%%%%%%%%%%%%%%%%%
 \scalebox{0.8}{
 \begin{tabular}{ c }
 %\hline  
  \bf{Tourniquet} \\
        \subfloat[Place TQ on Limb]          { \includegraphics[width=\skillFigTQSize\textwidth]{figures/skills_figure/M2_TQ_1.png} }
        \subfloat[Tighten TQ]                { \includegraphics[width=\skillFigTQSize\textwidth]{figures/skills_figure/M2_TQ_2.png} }
        \subfloat[Strap to Strap body]       { \includegraphics[width=\skillFigTQSize\textwidth]{figures/skills_figure/M2_TQ_3.png} }
        \subfloat[Tighten Windlass]          { \includegraphics[width=\skillFigTQSize\textwidth]{figures/skills_figure/M2_TQ_4.png} }
        \subfloat[Lock in Windlass]          { \includegraphics[width=\skillFigTQSize\textwidth]{figures/skills_figure/M2_TQ_5.png} }
        \subfloat[Secure Extra Strap]        { \includegraphics[width=\skillFigTQSize\textwidth]{figures/skills_figure/M2_TQ_6.png} }
        \subfloat[Secure Windlass]           { \includegraphics[width=\skillFigTQSize\textwidth]{figures/skills_figure/M2_TQ_7.png} }
        \subfloat[Mark Time]                 { \includegraphics[width=\skillFigTQSize\textwidth]{figures/skills_figure/M2_TQ_8.png} }
  \vspace{2mm}
  \\
  %
   \bf{Pressure Bandage} \\
        \subfloat[Apply Pressure]  { \includegraphics[width=\skillFigSixStepSize\textwidth]{figures/skills_figure/M3_PB_1.png} }
        \subfloat[Open Package]    { \includegraphics[width=\skillFigSixStepSize\textwidth]{figures/skills_figure/M3_PB_2.png} }
        \subfloat[Apply Dressing]  { \includegraphics[width=\skillFigSixStepSize\textwidth]{figures/skills_figure/M3_PB_3.png} }
        \subfloat[Wrap Dressing]   { \includegraphics[width=\skillFigSixStepSize\textwidth]{figures/skills_figure/M3_PB_4.png} }
        \subfloat[Secure Dressing] { \includegraphics[width=\skillFigSixStepSize\textwidth]{figures/skills_figure/M3_PB_5.png} }
        \subfloat[Apply Pressure ] { \includegraphics[width=\skillFigSixStepSize\textwidth]{figures/skills_figure/M3_PB_6.png} }
  \vspace{2mm}
  \\
  %
   \bf{Wound Dressing} \\
        \subfloat[Apply Pressure] { \includegraphics[width=\skillFigSixStepSize\textwidth]{figures/skills_figure/M4_WD_1.png} }
        \subfloat[Open Package]   { \includegraphics[width=\skillFigSixStepSize\textwidth]{figures/skills_figure/M4_WD_2.png} }
        \subfloat[Pack Wound]     { \includegraphics[width=\skillFigSixStepSize\textwidth]{figures/skills_figure/M4_WD_3.png} }
        \subfloat[Open Dressing]  { \includegraphics[width=\skillFigSixStepSize\textwidth]{figures/skills_figure/M4_WD_4.png} }
        \subfloat[Apply Dressing] { \includegraphics[width=\skillFigSixStepSize\textwidth]{figures/skills_figure/M4_WD_5.png} }
        \subfloat[Apply Pressure ]{ \includegraphics[width=\skillFigSixStepSize\textwidth]{figures/skills_figure/M4_WD_6.png} }
  \vspace{2mm}
  \\
  %
   \bf{Needle Chest Decompression} \\
        \subfloat[Clean Site]         { \includegraphics[width=\skillFigSixStepSize\textwidth]{figures/skills_figure/R19_NCD_1.png} }
        \subfloat[Prepare Needle Kit] { \includegraphics[width=\skillFigSixStepSize\textwidth]{figures/skills_figure/R19_NCD_2.png} }
        \subfloat[Locate Site]        { \includegraphics[width=\skillFigSixStepSize\textwidth]{figures/skills_figure/R19_NCD_3.png} }
        \subfloat[Insert Needle]      { \includegraphics[width=\skillFigSixStepSize\textwidth]{figures/skills_figure/R19_NCD_4.png} }
        \subfloat[Remove Needle]      { \includegraphics[width=\skillFigSixStepSize\textwidth]{figures/skills_figure/R19_NCD_5.png} }
        \subfloat[Tape Catheter]      { \includegraphics[width=\skillFigSixStepSize\textwidth]{figures/skills_figure/R19_NCD_6.png} }
  \\
  %
  \end{tabular}
}
  \caption{
         Example images for the first set of 4 skills.  Still-images were chosen to represent each step in a skill.
  }
  \label{tab:skills1}
\end{figure*}
%
%%^-------------------------------------------------------------------^

==> figures/skills_figure/skills2.tex <==
%%v-------------------------------------------------------------------v
%
\begin{figure*}[!htb]
\centering
%%%%%%%%%%%%%%%%%%%%%%%%%
 \scalebox{0.8}{
 \begin{tabular}{ c}
 %\hline  
  \bf{X-Stat} \\
        \subfloat[Open Package]            { \includegraphics[width=\skillFigFiveStepSize\textwidth]{figures/skills_figure/M5_XS_1.png} }
        \subfloat[Insert Applicator]       { \includegraphics[width=\skillFigFiveStepSize\textwidth]{figures/skills_figure/M5_XS_2.png} }
        \subfloat[Plunger into Applicator] { \includegraphics[width=\skillFigFiveStepSize\textwidth]{figures/skills_figure/M5_XS_3.png} }
        \subfloat[Push Plunger]            { \includegraphics[width=\skillFigFiveStepSize\textwidth]{figures/skills_figure/M5_XS_4.png} }
        \subfloat[Apply Pressure]          { \includegraphics[width=\skillFigFiveStepSize\textwidth]{figures/skills_figure/M5_XS_5.png} }
  \vspace{2mm}
  \\
  %
   \bf{Chest Seal} \\
        \subfloat[Apply Pressure]   { \includegraphics[width=\skillFigFiveStepSize\textwidth]{figures/skills_figure/R18_CS_1.png} }
        \subfloat[Open Package]     { \includegraphics[width=\skillFigFiveStepSize\textwidth]{figures/skills_figure/R18_CS_2.png} }
        \subfloat[Clean Wound]      { \includegraphics[width=\skillFigFiveStepSize\textwidth]{figures/skills_figure/R18_CS_3.png} }
        \subfloat[Remove Backing]   { \includegraphics[width=\skillFigFiveStepSize\textwidth]{figures/skills_figure/R18_CS_4.png} }
        \subfloat[Apply Chest Seal] { \includegraphics[width=\skillFigFiveStepSize\textwidth]{figures/skills_figure/R18_CS_5.png} }
  \vspace{2mm}
  \\
  %
  \bf{Nasal Pharyngeal Tube (NPA)} \\
        \subfloat[Size Tube]     { \includegraphics[width=\skillFigFiveStepSize\textwidth]{figures/skills_figure/A8_NPA_1.png} }
        \subfloat[Lube Tube]     { \includegraphics[width=\skillFigFiveStepSize\textwidth]{figures/skills_figure/A8_NPA_2.png} }
        \subfloat[Position Head] { \includegraphics[width=\skillFigFiveStepSize\textwidth]{figures/skills_figure/A8_NPA_3.png} }
        \subfloat[Insert Tube]   { \includegraphics[width=\skillFigFiveStepSize\textwidth]{figures/skills_figure/A8_NPA_4.png} }
        \subfloat[Check for airway compliance] { \includegraphics[width=\skillFigFiveStepSize\textwidth]{figures/skills_figure/A8_NPA_5.png} }
  \vspace{2mm}
  \\
  %
  \bf{Bag Valve Mask (BVM)} \\
        \subfloat[Open Package]       { \includegraphics[width=\skillFigFourStepSize\textwidth]{figures/skills_figure/R16_BVM_1.png} }
        \subfloat[Attach mask to bag] { \includegraphics[width=\skillFigFourStepSize\textwidth]{figures/skills_figure/R16_BVM_2.png} }
        \subfloat[Place mask]         { \includegraphics[width=\skillFigFourStepSize\textwidth]{figures/skills_figure/R16_BVM_3.png} }
        \subfloat[Squeeze bag]        { \includegraphics[width=\skillFigFourStepSize\textwidth]{figures/skills_figure/R16_BVM_4.png} }
  \\
  %  
  \end{tabular}
}
  \caption{
         Example images for the second set of 4 skills.  Still-images were chosen to represent each step in a skill.
  }
  \label{tab:skills2}
\end{figure*}
%
%%^-------------------------------------------------------------------^

==> figures/skills_figure/skills3.tex <==
%%v-------------------------------------------------------------------v
%
\begin{figure*}[h!t]
\begin{center}
%%%%%%%%%%%%%%%%%%%%%%%%%
 \scalebox{0.8}{
 \begin{tabular}{ c }
 %\hline  
  \bf{Tourniquet [M2]} \\
        \subfloat[Place TQ on Limb]          { \includegraphics[width=\skillFigTQSize\textwidth]{figures/skills_figure/M2_TQ_1.png} }
        \subfloat[Tighten TQ]                { \includegraphics[width=\skillFigTQSize\textwidth]{figures/skills_figure/M2_TQ_2.png} }
        \subfloat[Strap to Strap body]       { \includegraphics[width=\skillFigTQSize\textwidth]{figures/skills_figure/M2_TQ_3.png} }
        \subfloat[Tighten Windlass]          { \includegraphics[width=\skillFigTQSize\textwidth]{figures/skills_figure/M2_TQ_4.png} }
        \subfloat[Lock in Windlass]          { \includegraphics[width=\skillFigTQSize\textwidth]{figures/skills_figure/M2_TQ_5.png} }
        \subfloat[Secure Extra Strap]        { \includegraphics[width=\skillFigTQSize\textwidth]{figures/skills_figure/M2_TQ_6.png} }
        \subfloat[Secure Windlass]           { \includegraphics[width=\skillFigTQSize\textwidth]{figures/skills_figure/M2_TQ_7.png} }
        \subfloat[Mark Time]                 { \includegraphics[width=\skillFigTQSize\textwidth]{figures/skills_figure/M2_TQ_8.png} }
  \vspace{2mm}
  \\
  %
  \bf{X-Stat [M5]} \\
        \subfloat[Open Package]            { \includegraphics[width=\skillFigFiveStepSize\textwidth]{figures/skills_figure/M5_XS_1.png} }
        \subfloat[Insert Applicator]       { \includegraphics[width=\skillFigFiveStepSize\textwidth]{figures/skills_figure/M5_XS_2.png} }
        \subfloat[Plunger into Applicator] { \includegraphics[width=\skillFigFiveStepSize\textwidth]{figures/skills_figure/M5_XS_3.png} }
        \subfloat[Push Plunger]            { \includegraphics[width=\skillFigFiveStepSize\textwidth]{figures/skills_figure/M5_XS_4.png} }
        \subfloat[Apply Pressure]          { \includegraphics[width=\skillFigFiveStepSize\textwidth]{figures/skills_figure/M5_XS_5.png} }
  \vspace{2mm}
  \\
  %
  \bf{Bag Valve Mask (BVM) [R16]} \\
        \subfloat[Open Package]       { \includegraphics[width=\skillFigFourStepSize\textwidth]{figures/skills_figure/R16_BVM_1.png} }
        \subfloat[Attach mask to bag] { \includegraphics[width=\skillFigFourStepSize\textwidth]{figures/skills_figure/R16_BVM_2.png} }
        \subfloat[Place mask]         { \includegraphics[width=\skillFigFourStepSize\textwidth]{figures/skills_figure/R16_BVM_3.png} }
        \subfloat[Squeeze bag]        { \includegraphics[width=\skillFigFourStepSize\textwidth]{figures/skills_figure/R16_BVM_4.png} }
  \\
  % 
  \end{tabular}
}
  \caption{
         Example images of the most challenging 3 tasks.  Still images were chosen to represent each step in a task.
  }
  \label{tab:skills_chall}
\end{center}
\end{figure*}
%
%%^-------------------------------------------------------------------^
